Curriculum-Meta Learning for Order-Robust Continual Relation Extraction

Continual relation extraction is an important task that focuses on extracting new facts incrementally from unstructured text. Given the sequential arrival order of the relations, this task is prone to two serious challenges, namely catastrophic forgetting and order-sensitivity. We propose a novel curriculum-meta learning method to tackle the above two challenges in continual relation extraction. We combine meta learning and curriculum learning to quickly adapt model parameters to a new task and to reduce interference of previously seen tasks on the current task. We design a novel relation representation learning method through the distribution of domain and range types of relations. Such representations are utilized to quantify the difficulty of tasks for the construction of curricula. Moreover, we also present novel difficulty-based metrics to quantitatively measure the extent of order-sensitivity of a given model, suggesting new ways to evaluate model robustness. Our comprehensive experiments on three benchmark datasets show that our proposed method outperforms the state-of-the-art techniques. The code is available at the anonymous GitHub repository: https://github.com/wutong8023/AAAI_CML.

==> sec3-order.tex <==

\section{Task Order-Sensitivity in Continual Learning}\label{sec:order}

\begin{itemize}
\item The average forgetting rate per task after $k$ time steps,  $Fr^j_{avg}$, which is defined in Eq.(\ref{eq-fravg})
\item The error bound $EB$ of $Acc_a$, $Acc_w$, which is defined in Eq.(\ref{eq-eb}). 
\end{itemize}

% \hl{(i) define continual learning, (ii) explain the concept of order sensitivity in continual learning, (iii) explain what leads to order sensitivity and difficulty of a task in a given sequence of tasks is whether there are similar tasks before the task in a given sequence, (iv) mention the impact of  order sensitivity in (a) robust evaluation of continual learning algorithms based on multiple sequences of tasks (to prevent the bias of particular sequence of tasks), (b) we make use of the task similarity to invent a new continual learning algorithm which makes use of this notion. }
Continual learning is also known as lifelong learning, in which there is a sequence of $K$ tasks $\{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_K\}$. Each task $\mathcal{T}_k$ is a conventional supervised learning task, with each task represented as $\{(x^{(i)}, y^{(i)})\}$ and partitioned as $\{\mathcal{D}^{train}, $ $\mathcal{D}^{valid}, \mathcal{D}^{test}\}$. Due to the limited storage capacity, the model $f_\theta(.)$ can only view the training data of the current task $T_k$ and is trained with a learner $l(f_\theta(x), y)$, with no access to the previous or following tasks. The goal of continual learning is to train the model $f_\theta(.)$ such that it continually learns new tasks while avoiding forgetting the previously learned tasks, i.e.\ the \emph{catastrophic forgetting} problem. The performance of the model $f_\theta(.)$ is evaluated with a measure averaged on the test sets of \hl{$\{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_{K-1}\}$} \yf{or just `the sequence of tasks'}. Practically, to improve the model's performance on previous tasks, the learner is typically allowed to maintain and observe a memory $\mathcal{M}$ of prototype instances from previous tasks.

It has been observed that the order of tasks may have a significant impact on a model's final performance in continual learning, which is referred to as the \emph{order-sensitivity} problem in the literature~\cite{CITE}. To counter the effect of order-sensitivity, one can try several random sequences of tasks and use the average performance for comparison purposes. However, in real application scenarios of continual relation extraction, such as knowledge base construction and population, such an approach is infeasible, as the order of tasks cannot be pre-determined. Thus, the problem of order-sensitivity leads to uncontrollable and uncertain quality of the extracted knowledge. 

We postulate that order-sensitivity is an effect of the \emph{difficulty} of tasks, which can be defined as the similarity between tasks in a sequence. \yf{Mention that this postulation is validated in Sec. 6.7?}

In this section, we first formulate a robust performance metric for order-sensitivity that measures the average rate of forgetting of multiple sequences. 
We also propose a function that estimates the difficulty of a given task, which is calculated from its similarity with the other tasks in a sequence, where the pairwise task similarity is defined on the embedding of the two tasks. 

\subsection{The Evaluation Metrics for Order-Sensitivity}
To comprehensively understand the of order-sensitivity issue and analyze task-specific performances, We introduce two metrics for the overall performance and the task-specific performance respectively.

\subsubsection{The Overall Metric for Order-sensitivity.}
We introduce the \emph{error bound}, $EB$, as a new metric to evaluate the overall model performance regarding order-sensitivity.
\begin{equation}
EB := Z_{\frac{\alpha}{2}}\times\frac{\delta}{\sqrt{n}},
\label{eq-eb}
\end{equation}
where $Z_{\frac{\alpha}{2}}$ is the confidence coefficient of confidence level $\alpha$, and $\delta$ is the standard deviation of accuracy obtained from $n$ distinct task permutations. Note that a model with a lower error bound shows better robustness and less order-sensitivity for the input sequences.

\subsubsection{The Task-specific Metric for Order-sensitivity.}
we introduce the \emph{average forgetting rate} for task $j$ after $k$ \hl{time steps} \yf{`tasks'?}, $Fr^j_{avg}$, as a new metric to evaluate task-specific model performance on order-sensitivity. 
\begin{equation}
Fr^j_{avg}:=\frac{1}{k-1}\sum^{k-1}_{i=1}\frac{\overline{acc}^j_{i+1}-\overline{acc}^j_{i}}{\overline{acc}^j_{i}},
\label{eq-fravg}
\end{equation}
where $\overline{acc}^j_{i}$ is the model's average performance on a specific task $\mathcal{T}_j$ when it appears in the $i$th position of distinct task permutations:
\begin{equation}
\overline{acc}^j_{i} := \frac{1}{(J-1)!}\sum_{\pi \in \Pi_{[1,\ldots,J]} \text{ st } \pi_i = j} acc_{i}(\pi) 
\end{equation}
where $acc_{i}(\pi)$ is the final accuracy on task $\mathcal{T}_i$ of the model trained on the permutation $\pi$, $\Pi_{[1,..,J]}$ is the set of all permutations of the tasks $\{\mathcal{T}_1,\ldots,\mathcal{T}_J\}$, and $\pi_i$ is the index of Task $T_i$ of the sequence.  We note that the number of all permutations in which task $\mathcal{T}_i$ is fixed at position $j$ is $(J-1)!$. Of course we may not be able to exactly compute $\overline{acc}^j_{f, i}$ as the size of possible tasks persmutations grows exponentially. Therefore, we estimate this quantity by Monte Carlo sampling of some permutations.

\subsubsection{Task Difficulty as the Cause of Order-sensitivity.}
Intrinsically, order-sensitivity is caused by a model's inability to guarantee optimal performance for all previous tasks. However, from the perspective of experiments, order-sensitivity is closely related to the unbalanced forgetting rate (or the unbalanced difficulty) of different tasks, where we assume that task difficulty is due to the interactions between semantically similar relations in an observed task sequence. 

To formalize this intuition, we define a difficulty estimation function based on the semantic embeddings of relations in each task. Given a set of tasks $\mathcal{T}_i$ in $\{\mathcal{T}_1, \mathcal{T}_2, ..., \mathcal{T}_K\}$, the difficulty of task $\mathcal{T}_i$ is defined as:
\begin{equation}
    Dl_i := \frac{1}{K-1}\sum_{j=1}^{K-1}S_i^j,
    \label{eq-whole_diff}
\end{equation}
where $K$ is the number of tasks, and $S_j^i$ is the similarity score between tasks $\mathcal{T}_i$ and  $\mathcal{T}_j$, which is defined as the average similarity among relation pairs from two tasks:
\begin{equation}
    S_i^j := \frac{1}{M\times N}\sum_{m=1}^{M}\sum_{n=1}^{N}s_m^n,
    \label{eq-Similarity}
\end{equation}
where $M$ and $N$ are the numbers of relations in each task respectively, and  $s_m^n$ calculates the Cosine similarity between two relations:
\begin{equation}
    s_m^n := \cos(emd_m, emd_n),
\end{equation}
where $emd$ represents the semantic embedding of each relations. 

\subsubsection{The Impact of Order-sensitivity.}
Order-sensitivity is a robust evaluation of continual learning algorithms based on multiple sequences of tasks (to prevent the bias of particular sequence of tasks).

Based on the Pearson's correlation coefficient between the expected difficulty gained by Eq.(\ref{eq-whole_diff}) and the average forgetting rate gained by Eq.(\ref{eq-Similarity}) of each tasks. There is positive correlation between the average forgetting rate of tasks and the predicted difficulty based on semantic similarity, indicating the pretrained semantic-similarity would be an important information to alleviate the catastrophic-forgetting and the order-sensitivity.
 
This difficulty estimation function $Dl_i$ is employed in our curriculum-meta learning method, which is described in Section~\ref{sec:method}, to design an effective curriculum construction strategy to alleviate the order-sensitivity issue. 
We empirically validate our proposed metrics and study the effectiveness of our difficulty-guided curriculum-meta learning method in Section~\ref{sec:experments}



% (a) robust evaluation of continual learning algorithms based on multiple sequences of tasks (to prevent the bias of particular sequence of tasks), (b) we make use of the task similarity to invent a new continual learning algorithm which makes use of this notion. }


% Meta learning部分


% 1.
% 主框架图部分：
% 叙述任务的执行流程；
% 介绍task任务输入的设定
% 介绍memory的作用
% 介绍训练以及测试阶段的功能


% 2. meta learning的形式化定义



